Sparse Compressed Spiking Neural Network Accelerator for Object Detection

Spiking neural networks (SNNs), which are inspired by the human brain, have recently gained popularity due to their relatively simple and low-power hardware for transmitting binary spikes and highly sparse activation maps. However, because SNNs contain extra time dimension information, the SNN accelerator will require more buffers and take longer to infer, especially for the more difficult high-resolution object detection task. As a result, this paper proposes a sparse compressed spiking neural network accelerator that takes advantage of the high sparsity of activation maps and weights by utilizing the proposed gated one-to-all product for low power and highly parallel model execution. The experimental result of the neural network shows 71.5$\%$ mAP with mixed (1,3) time steps on the IVS 3cls dataset. The accelerator with the TSMC 28nm CMOS process can achieve 1024$\times$576@29 frames per second processing when running at 500MHz with 35.88TOPS/W energy efficiency and 1.05mJ energy consumption per frame.

==> tables/table-classopt.tex <==
\begin{table}[h]
\centering
% [] 顯示在 list of tables 的文字
% {} 顯示在表格上方的文字
\caption[Class options provided by thesis.cls]{Class options provided by thesis.cls}
\label{table:clsoptions}
\begin{tabular}{lll}
\toprule[1.1pt]
                      & Options   & Description\\
\midrule[1.1pt]
\multirow{2}{*}{論文類型} & master    & 碩士論文 (default)\\
                      & phd       & 博士論文\\
\midrule
\multirow{3}{*}{論文格式} & draft     & 初稿 (default)\\
                      & final     & 終稿\\
                      & review    & 只顯示內文,參考文獻,與附錄\\
\midrule
\multirow{2}{*}{語言}   & en        & 英文章節編號與標題 (default)\\
                       & zh        & 中文章節編號與標題\\
\midrule
\multirow{2}{*}{列印}   & oneside   & 單面列印 (default)\\

                        & twoside   & 雙面列印\\
\midrule
浮水印                   & watermark & \begin{tabular}[c]{@{}l@{}}review mode 不顯示\\ draft mode 顯示 ``DRAFT" 字樣\\ final mode 顯示指定的浮水印\end{tabular} \\
\midrule
裝訂                    & binding   & \begin{tabular}[c]{@{}l@{}} 在頁面左側預留 1cm 的裝訂空間\\ (enabled by default under final mode)\end{tabular}\\
\bottomrule[1.1pt]
\end{tabular}
\end{table}


==> tables/table-files.tex <==
\begin{table}[h]
\centering
% [] 顯示在 list of tables 的文字
% {} 顯示在表格上方的文字
\caption[檔案位置]{檔案位置}
\label{table:pages}
\begin{tabular}{@{}ll@{}}
\toprule
     & 位置                      \\ \midrule
中文摘要 & abs/abstract\_zh.tex    \\
英文摘要 & abs/abstract\_en.tex    \\
誌謝   & ack/ack.tex             \\
題獻頁  & ack/dedication.tex      \\
自傳   & author/cv.tex           \\
著作目錄 & author/publications.tex \\ \bottomrule
\end{tabular}
\end{table}
